cViL: Cross-Lingual Training of Vision-Language Models using Knowledge Distillation

Vision-and-language tasks are gaining popularity in the research community, but the focus is still mainly on English. We propose a pipeline that utilizes English-only vision-language models to train a monolingual model for a target language. We propose to extend OSCAR+, a model which leverages object tags as anchor points for learning image-text alignments, to train on visual question answering datasets in different languages. We propose a novel approach to knowledge distillation to train the model in other languages using parallel sentences. Compared to other models that use the target language in the pretraining corpora, we can leverage an existing English model to transfer the knowledge to the target language using significantly lesser resources. We also release a large-scale visual question answering dataset in Japanese and Hindi language. Though we restrict our work to visual question answering, our model can be extended to any sequence-level classification task, and it can be extended to other languages as well. This paper focuses on two languages for the visual question answering task - Japanese and Hindi. Our pipeline outperforms the current state-of-the-art models by a relative increase of 4.4% and 13.4% respectively in accuracy.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> images/tsne.tex <==
\begin{figure*}[ht]

% \noindent
\begin{minipage}{0.33\textwidth}
  \centering
  \subfigure[Output embeddings of the textual tokens by teacher and student model.\label{fig:tsne-text}]{
    % \includegraphics[width=.7\textwidth]{images/yoda.jpeg}
    \includegraphics[width=0.9\textwidth]{tsne/en-ja_text[cropped].png}
  }
\end{minipage} % This must go next to `\end{minipage}`
\begin{minipage}{0.33\textwidth}
  \centering
  \subfigure[Output embeddings of the image tokens by teacher and student model.\label{fig:tsne-image}]{
    % \includegraphics[width=.7\textwidth]{images/yoda.jpeg}
    \includegraphics[width=0.9\textwidth]{tsne/en-ja_image[cropped].png}
  }
\end{minipage} 
\begin{minipage}{0.33\textwidth}
  \centering
  \subfigure[Alignment between image and textual embeddings output by our student model.\label{fig:tsne-ja}]{
    % \includegraphics[width=.7\textwidth]{images/yoda.jpeg}
    \includegraphics[width=0.9\textwidth]{tsne/ja_text-image[cropped].png}  
  }
\end{minipage}%
\caption{2D visualization of the output embeddings of the teacher and student model using t-SNE. The points from the same object class share the same color.}
\label{fig:tsnes}
\end{figure*}

==> tables/table_ablations.tex <==
\begin{table}[!ht]
\begin{center}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{Accuracy} \\%& \textbf{BLEU} \\
\midrule
% \modelone & $ABC$ & ?\\
\modeltwo & $\textbf{35.72}$ \\%& ?\\
\modeltwo (w/o classification token distillation) & $35.58$\\% & ?\\
\modeltwo (w/o code-mixed distillation) & $35.57$\\% & ?\\
\modeltwo (w/o image tokens distillation) & $35.38$ \\%& ?\\
\modeltwo (w/o object tags distillation) & $35.19$ \\%& ?\\
\modeltwo (w/o intermediate layers distillation) & $34.55$ \\%& ?\\
\modelbase & $33.75$\\% & ?\\
\bottomrule
\end{tabular}
% }%
\end{center}
\caption{Ablation studies of the various distillation objectives.}
\label{tab:ablations}
\end{table}

==> tables/table_classes.tex <==
\begin{table}[!ht]

% \noindent\begin{minipage}{.5\columnwidth}
  \centering
  \subtable[Class-wise scores for the different question types in the test set of Japanese dataset. We identify the question type by checking the presence of each question word.]{
    % \includegraphics[width=.7\textwidth]{images/yoda.jpeg}
    \input{tables/table_classes_jap}
  }
% \end{minipage}% This must go next to `\end{minipage}`
% \begin{minipage}{.5\textwidth}
  \centering
  \subtable[Class-wise scores for the different question types in the test set of the VQA dataset.]{
    % \includegraphics[width=.7\textwidth]{images/yoda.jpeg}
    \input{tables/table_classes_hin}
  }
% \end{minipage}%
\caption{Performance of our systems on the various question types in the dataset.}
\label{tab:classes}
\end{table}

% \begin{table}[!ht]
% \setlength{\fboxsep}{0pt}
% \fbox{
% \begin{minipage}{.5\textwidth}
% \subtable[Picture 1]{\includegraphics[width=.9\textwidth]{images/yoda.jpeg} \label{fig:1}}%
% \end{minipage}}%
% \fbox{
% \begin{minipage}{.5\textwidth}
% \subtable[Picture 2]{\includegraphics[width=.9\textwidth]{images/yoda.jpeg} \label{fig:2}}%
% \end{minipage}}%
%   \caption{TODO}
% \end{table}

==> tables/table_classes_hin.tex <==
\begin{tabular}{lc}
\toprule
\textbf{Question type} & \textbf{Accuracy} \\
\midrule
Yes / No & $86.99$ \\
Number & $58.18$ \\
Other & $63.65$ \\
Overall & $72.65$ \\
\bottomrule
\end{tabular}

==> tables/table_classes_jap.tex <==
\begin{tabular}{lc}
\toprule
\textbf{Question type} & \textbf{Accuracy} \\
\midrule
\textit{nani} (what) & $38.21$ \\
\textit{dare} (who) & $35.40$ \\
\textit{doko} (where) & $23.74$ \\
\textit{donna} (what kind) & $36.10$ \\
\textit{dorekurai} (how much) & $33.17$ \\
\textit{dou} (how) & $32.24$ \\
\textit{itsu} (when) & $63.25$ \\
\textit{ikutsu} (how many) & $29.22$ \\
\textit{naze} (why) & $11.44$ \\
\bottomrule
\end{tabular}

==> tables/table_hin_results.tex <==
% \begin{table}[!h]
% \begin{center}
\begin{threeparttable}
\begin{tabular}{lc}
\toprule
\textbf{Model} & \textbf{Accuracy} \\
\midrule
BUTD\textsuperscript{*}~\citep{gupta-etal-2020-unified} & $60.15$ \\
Bi-linear Attention\textsuperscript{*}~\citep{gupta-etal-2020-unified} & $62.50$ \\
Multimodal Fusion\textsuperscript{*}~\citep{gupta-etal-2020-unified} & $64.51$ \\
% \modeltwo & $\textbf{73.12}$ \\
\midrule
% \modelbase & $68.14$ \\
% \modeltwo & $\textbf{71.74}$ \\
\modelbase & $67.71$ \\
\modeltwo & $\textbf{72.65}$ \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item [*] They use the translated version of VQA 1.0, instead of VQA 2.0. 
% \item \color{blue}{Fixed citations in the models?}
% \item \color{red}{Add results for VQA 1.0 val set}

\item [] 
\end{tablenotes}
\end{threeparttable}
% \end{center}
% \caption{Evaluation results on the Hindi version of VQA 2.0 dataset.}
% \label{tab:hin_results}

% \end{table}

==> tables/table_ir_results.tex <==
% \begin{table}[!h]
% \begin{center}
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{EN} & \textbf{ZH} & \textbf{JA} & \textbf{Meta-Ave} \\
\midrule
EmbN~\citep{?} & 	$76.8$ & 	$73.2$ & 	$73.5$ & 	$74.5$ \\
PAR.EmbN~\citep{?} & 	$78.3$ & 	$76.0$ & 	$74.8$ & 	$?$ \\
S-LIWE~\citep{?} & 	$80.9$ & 	$73.6$ & 	$70.0$ & 	$?$ \\
MULE~\citep{?} & 	$79.0$ & 	$75.9$ & 	$75.6$ & 	$?$ \\
SMALR~\citep{?} & 	$81.5$ & 	$77.5$ & 	$76.7$ & 	$?$ \\
UNITER~\citep{?} & $0$  & $0$  & $0$  & $0$  \\
M\textsuperscript{3}P~\citep{?} & $88.7$  & $86.2$  & $87.9$  & $?$  \\
UC\textsuperscript{2}~\citep{zhou2021uc} & $88.1$  & $89.8$  & $87.5$  & $?$  \\
\midrule
\modelbase & 	$79.0$ & 	$75.9$ & 	$75.6$ & 	$?$ \\
\modelone & 	$79.0$ & 	$75.9$ & 	$75.6$ & 	$?$ \\
\modeltwo & 	$79.0$ & 	$75.9$ & 	$75.6$ & 	$?$ \\
\bottomrule
\end{tabular}
\begin{tablenotes}
% \item [*] They use different train / dev / test splits.
% \item [] 
\end{tablenotes}
\end{threeparttable}
% \end{center}
% \caption{Evaluation results on VG VQA Japanese dataset.}
% \label{tab:jap_results}

% \end{table}



==> tables/table_jap_results.tex <==
% \begin{table}[!h]
% \begin{center}
\begin{adjustbox}{max width=\columnwidth}
\begin{threeparttable}
\begin{tabular}{lcc}
\toprule
% \textbf{Model} & \textbf{Accuracy} & \textbf{BLEU} \\
\textbf{Model} & \textbf{Accuracy} & \textbf{BLEU} \\
\midrule
PCATT\textsuperscript{*}~\citep{C18-1163} & $19.2$ & - \\
UNITER\textsubscript{CC}~\citep{ChenLYK0G0020,zhou2021uc} & $22.7$ & $11.8$ \\
UC\textsuperscript{2}~\cite{zhou2021uc} & $34.2$ & $26.8$ \\
\midrule
\modelbase & $33.75$ & $32.5$ \\
\modelone & $34.93$ & $\textbf{33.6}$ \\
\modeltwo & $\textbf{35.72}$ & $33.1$ \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item [*] They use different train / dev / test splits.
% \item [] \textcolor{red}{Add English as well?}
\item [] 
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
% \end{center}
% \caption{Evaluation results on VG VQA Japanese dataset.}
% \label{tab:jap_results}

% \end{table}

==> tables/table_results.tex <==
\begin{table}[ht]

% \noindent
% \begin{minipage}{.5\columnwidth}
%   \centering
  \subtable[Test set of the Japanese Visual Genome VQA dataset.\label{tab:jap_results}]{
    % \includegraphics[width=.7\textwidth]{images/yoda.jpeg}
    \input{tables/table_jap_results}
  }
% \end{minipage}% This must go next to `\end{minipage}`
% \begin{minipage}{.5\columnwidth}
%   \centering
  \subtable[Hindi version of test-dev set of VQA 2.0 dataset.\label{tab:hin_results}]{
    % \includegraphics[width=.7\textwidth]{images/yoda.jpeg}
    \input{tables/table_hin_results}
  }
% \end{minipage}%
\caption{Performance of our systems on the two VQA datasets we consider.}
\end{table}
